FoveaSPAD: Exploiting Depth Priors for Adaptive and Efficient Single-Photon 3D Imaging

Fast, efficient, and accurate depth-sensing is important for safety-critical applications such as autonomous vehicles. Direct time-of-flight LiDAR has the potential to fulfill these demands, thanks to its ability to provide high-precision depth measurements at long standoff distances. While conventional LiDAR relies on avalanche photodiodes (APDs), single-photon avalanche diodes (SPADs) are an emerging image-sensing technology that offer many advantages such as extreme sensitivity and time resolution. In this paper, we remove the key challenges to widespread adoption of SPAD-based LiDARs: their susceptibility to ambient light and the large amount of raw photon data that must be processed to obtain in-pixel depth estimates. We propose new algorithms and sensing policies that improve signal-to-noise ratio (SNR) and increase computing and memory efficiency for SPAD-based LiDARs. During capture, we use external signals to \emph{foveate}, i.e., guide how the SPAD system estimates scene depths. This foveated approach allows our method to ``zoom into'' the signal of interest, reducing the amount of raw photon data that needs to be stored and transferred from the SPAD sensor, while also improving resilience to ambient light. We show results both in simulation and also with real hardware emulation, with specific implementations achieving a 1548-fold reduction in memory usage, and our algorithms can be applied to newly available and future SPAD arrays.

==> Figs/FoveationResults_figure.tex <==
% FileNames
\newcommand{\Fa}{00034}
\newcommand{\Fb}{00315}
\newcommand{\Fc}{00355}
\newcommand{\Fd}{00431}
\newcommand{\Fe}{01170}
% FileSubnames
\newcommand{\SubDS}{_DS}
\newcommand{\SubDSD}{_DSDepths}
\newcommand{\SubDSE}{_DSDepthsErrors}
\newcommand{\SubDSGS}{_DSDepthsGS}
\newcommand{\SubGTD}{nyu_depths}
\newcommand{\SubGTRGB}{nyu_rgb}
\newcommand{\SubFS}{_fullsim}
\newcommand{\SubFSE}{_fullsimErrors}
\newcommand{\SubFSGS}{_histGS}
\newcommand{\SubMD}{_memDepths}
\newcommand{\SubME}{_memErorrs}
\newcommand{\SubMGS}{_memGS}
\newcommand{\SubMono}{monocular_depth}

%Overleaf Paths, A = 60 B = 125 C = 250
\newcommand{\OPA}{Figs/S1_experiments/win60}
\newcommand{\OPB}{Figs/S1_experiments/win125}
\newcommand{\OPC}{Figs/S1_experiments/win250}
\newcommand{\OPGTRGB}{Figs/S1_experiments/RGB/}
\newcommand{\OPGTD}{Figs/S1_experiments/GT_D/}
\newcommand{\OPMono}{Figs/S1_experiments/Mono_D/}


\newcommand*{\incl}[1]{%
    {
    \includegraphics[width=0.143\linewidth,valign=m]{#1}
    }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure*}[t!]
\setlength{\tabcolsep}{0.01cm}
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ROW 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{tabular}{c c c c b{0.15cm}  c c p{1.5cm}}
        \textbf{NYUv2 RGB} & \textbf{NYUv2 Depth} & \textbf{Monocular}  & \textbf{Limited Bins (N$^\prime$)} & {} & \textbf{Memory Fovea} & \textbf{Depth Fovea} & {}\\
%%%%%%%%%%%%% 1ST SET %%%%%%%%%%%%        
        \incl{\OPGTRGB\Fd nyu_rgb.pdf} & 
        \incl{\OPGTD\Fd nyu_depths.pdf} & 
        \incl{\OPMono\Fd monocular_depth.pdf} &  
        \incl{\OPA/16Bin/\Fd\SubDS.pdf} & 
        {} & 
        \incl{\OPA/16Bin/\Fd\SubMD.pdf} & 
        \incl{\OPA/16Bin/\Fd\SubDSD.pdf} & 
        \textbf{\small{M=1/16N  N$^\prime$ = 16}}\\

        \incl{\OPGTRGB\Fc nyu_rgb.pdf} & 
        \incl{\OPGTD\Fc nyu_depths.pdf} & 
        \incl{\OPMono\Fc monocular_depth.pdf} &  
        \incl{\OPB/16Bin/\Fc\SubDS.pdf} & 
        {} & \incl{\OPB/16Bin/\Fc\SubMD.pdf} 
        & \incl{\OPB/16Bin/\Fc\SubDSD.pdf} & 
        \textbf{\normalsize{M=1/8N N$^\prime$ = 16}}\\

%%%%%%%%%%%%%% 2ND SET %%%%%%%%%%
        \incl{\OPGTRGB\Fd nyu_rgb.pdf} & 
        \incl{\OPGTD\Fd nyu_depths.pdf} & 
        \incl{\OPMono\Fd monocular_depth.pdf} &  
        \incl{\OPA/64Bin/\Fd\SubDS.pdf} & 
        {} & 
        \incl{\OPA/64Bin/\Fd\SubMD.pdf} & 
        \incl{\OPA/64Bin/\Fd\SubDSD.pdf} & 
        \textbf{\normalsize{M=1/16N N$^\prime$ = 64}}\\

        \incl{\OPGTRGB\Fc nyu_rgb.pdf} & 
        \incl{\OPGTD\Fc nyu_depths.pdf} & 
        \incl{\OPMono\Fc monocular_depth.pdf} &  
        \incl{\OPB/64Bin/\Fc\SubDS.pdf} & 
        {} & 
        \incl{\OPB/64Bin/\Fc\SubMD.pdf} & 
        \incl{\OPB/64Bin/\Fc\SubDSD.pdf} & 
        \textbf{\normalsize{M=1/8N N$^\prime$ = 64}}\\

    \end{tabular}



 \caption{\textbf{Qualitative Comparison on NYUv2} Our memory and depth foveation techniques produce quality depth reconstructions with a fraction of the memory usage. Each row consists of the NYUv2 ground truth images, the monocular depth output from ZoeDepth, a simulated SPAD output with N$^\prime$ bins, and our foveation techniques. The rows show different combinations of M and N$^\prime$, where M is the number of bins in the foveated histograms, and N$^\prime$ is the limited number of bins used for depth foveation. Monocular estimation is just one method of obtaining a depth prior in a class of methods, in sec. \ref{sec:6opflow} and sec. \ref{sec:hardware} we show two more methods.} 
 % there are 3 algs, we show one
 \label{fig:compare_wSize_DS}
\end{figure*}

==> Figs/local_errors_depth.tex <==
\begin{table*}
\begin{center}
%\centering
\centerline{
% \resizebox{1\columnwidth}{!}{
\tabcolsep=0.11cm
\begin{tabular}{c|cccc|ccc}
\toprule
\textbf{\small{Depth Resolution}} & \textbf{\small{RMSE}}  & \textbf{\small{Limited}} &\textbf{log}$\bm{_{10}}$ &\textbf{REL} & $\bm{\delta_1}$ & $\bm{\delta_2}$ & $\bm{\delta_3}$ \\
(Num Bins, Mem. Use) & (m) & \textbf{\small{RMSE}} (m) & (m) & (\%) & (\%)       & (\%)       & (\%)       \\
\hline 
16, 1/16 & 0.235 &  & 0.0173 &  3.60 & 96.55 & 98.96 & 99.48 \\
32, 1/16 & 0.211 &  & 0.0119 &  2.41 & 97.1 & 99.14 & 99.55 \\
64, 1/16 & 0.2238 &  & 0.012 &  2.42 & 96.44 & 99.01 & 99.54 \\
16, 1/8 & 0.201 &   & 0.018 &  4.18 & 97.87 & 99.26 & 99.71 \\
32, 1/8 & 0.184 &   & 0.011 & 2.54 & 98.1 & 99.38 & 99.77 \\
64, 1/8 & 0.121 &   & 0.0064 &  4.81 & 99.98 & 99.99 & 99.99 \\
16, 1/8 & 0.221 &   & 0.0326 &  7.14 & 98.77 & 99.6 & 99.82 \\
32, 1/8 & 0.166 &  & 0.015 &  3.55 & 99.15 & 99.59 & 99.82 \\
64, 1/8 & 0.145 &   & 0.0087 &  1.95 & 99.01 & 99.52 & 99.78 \\

\bottomrule
\end{tabular}
}
\end{center}

\vspace{-2mm}
\caption{\textbf{Depth Foveation Evaluation - Local Scale}}
\label{table:fovea_eval}
\end{table*}

==> Figs/local_errors_mem.tex <==
\begin{table*}
\caption{\textbf{Memory and Depth Foveation Evaluation - Local Scale} This table shows a quantitative comparison of RMSE and depth inlier metrics for different depth and memory foveation strategies for the NYUv2 dataset and a monocular estimation prior. For each memory fovation fraction, we vary the number of histogram bins in the foveated sub-window to achieve depth foveation.}
\label{table:fovea_eval}
\begin{center}
%\centering
% \resizebox{1\columnwidth}{!}{
\tabcolsep=0.11cm
\begin{tabular}{|c|ccc|ccc||c|cccc|ccc|}
% \toprule
\hline

\textbf{\small{Mem. Usage}}  & \textbf{\small{RMSE}}  &\textbf{log}$\bm{_{10}}$ &\textbf{REL} & $\bm{\delta_1}$ & $\bm{\delta_2}$ & $\bm{\delta_3}$ & \textbf{\small{Depth Res.}}  & \textbf{\small{RMSE}} & \textbf{\small{Lim. Bins}} &\textbf{log}$\bm{_{10}}$ &\textbf{REL} & $\bm{\delta_1}$ & $\bm{\delta_2}$ & $\bm{\delta_3}$ \\
             (Fraction)  & (m) & (m) & (\%) & (\%)  & (\%) & (\%) &(Num. Bins)  & (m) & \textbf{\small{RMSE}} (m) &(m) & (\%) & (\%)  & (\%) & (\%)   \\
\hline 
1/16  & 0.211 & 0.0106  & 2.11 & 97.07  & 99.13 & 99.55 &
16  & 0.235  & 0.504 & 0.0173 &  3.60 & 96.55 & 98.96 & 99.48 \\
 &  &  &  &  &  &  &
32   & 0.211 & 0.250 & 0.0119 &  2.41 & 97.1 & 99.14 & 99.55 \\
 &  &  &  &  &  &  &
64 & 0.211 & 0.121 & 0.012 &  2.42 & 96.44 & 99.01 & 99.54 \\

1/8 & 0.151 & 0.005 & 1.09 & 98.36 & 99.42 & 99.79 & 
16 & 0.201 & 0.509 & 0.018 &  4.18 & 97.87 & 99.26 & 99.71 \\
 &  &  &  &  &  & &    
32 & 0.184 & 0.250 & 0.011 & 2.54 & 98.1 & 99.38 & 99.77 \\
 &  &  &  &  &  & &  
64  & 0.12 &  0.121 & 0.0064 &  4.81 & 99.98 & 99.99 & 99.99 \\

1/4 & 0.117 & 0.0032 & 6.86 & 99.24 & 99.57 & 99.79&  
16  & 0.221& 0.501  & 0.0326 &  7.14 & 98.77 & 99.6 & 99.82 \\
  & &  &  &  &  & &  
32  & 0.166 & 0.2497 & 0.015 &  3.55 & 99.15 & 99.59 & 99.82 \\
  &  &  &  & &  & &  
64  & 0.145 & 0.123 & 0.0087 &  1.95 & 99.01 & 99.52 & 99.78 \\
\hline
% \bottomrule
\end{tabular}

\end{center}
\end{table*}

==> Figs/opticalFlow_table.tex <==
\begin{table}
\caption{\textbf{Optical-Flow Driven Foveation - Quantitative Comparison }}
\label{table:optflow_fovea_eval}
\begin{center}
%\centering
% \resizebox{1\columnwidth}{!}{
\tabcolsep=0.11cm
\begin{tabular}{|c|cc||c|ccc|}
% \toprule
\hline

\textbf{\small{Memory}}  & \textbf{\small{RMSE}}   &\textbf{SSIM} & \textbf{\small{Z Res.}}  & \textbf{\small{RMSE}} & \textbf{\small{Lim. Bins}} &\textbf{SSIM}  \\
             (Fraction)  & (m)  &  & (Bins)  & (m) & \textbf{\small{RMSE}} (m)  &  \\
\hline 
1/16  & 0.181  & 0.722  &
16  & 21.27  & 25.929  &  0.719  \\


1/8 & 0.202  & 0.722 &  
16 & 20.842  & 25.929 & 0.416 \\
 % &  &  &  &  &  & &    
% 32 & 0.184 & 0.250 & 0.011 & 2.54 \\
%  &  &  &  &  &  & &  
% 64  & 0.12 &  0.121 & 0.0064 &  4.81 \\

1/4 & 0.289 & 0.722 &  
16  & 21.261 &  25.929  & 0.294\\
%   & &  &  &  &  & &  
% 32  & 0.166 & 0.2497 & 0.015 &  3.55 \\
%   &  &  &  & &  & &  
% 64  & 0.145 & 0.123 & 0.0087 &  1.95 \\
\hline
% \bottomrule
\end{tabular}

\end{center}
\end{table}
